Adaptive Stochastic Weight Averaging

Ensemble models often improve generalization performances in challenging tasks. Yet, traditional techniques based on prediction averaging incur three well-known disadvantages: the computational overhead of training multiple models, increased latency, and memory requirements at test time. To address these issues, the Stochastic Weight Averaging (SWA) technique maintains a running average of model parameters from a specific epoch onward. Despite its potential benefits, maintaining a running average of parameters can hinder generalization, as an underlying running model begins to overfit. Conversely, an inadequately chosen starting point can render SWA more susceptible to underfitting compared to an underlying running model. In this work, we propose Adaptive Stochastic Weight Averaging (ASWA) technique that updates a running average of model parameters, only when generalization performance is improved on the validation dataset. Hence, ASWA can be seen as a combination of SWA with the early stopping technique, where the former accepts all updates on a parameter ensemble model and the latter rejects any update on an underlying running model. We conducted extensive experiments ranging from image classification to multi-hop reasoning over knowledge graphs. Our experiments over 11 benchmark datasets with 7 baseline models suggest that ASWA leads to a statistically better generalization across models and datasets

==> tables/fb_yago.tex <==
% CD : Firstly report all the results here
% CD: Later move the results from here to appendix
% CD: Keep only the most important onces here



% \begin{table*}
% \caption{Link prediction results on the train, validation and test splits of FB15K-237 and YAGO3-10. 
% Bold results indicate the best results.
% Num epochs 512, dim 32, batch size 1024 Adam with lr 0.1.}
% \label{table:fb15k_yago}
% \centering
% \small
% \begin{tabular}{l c c c c c c c c c}
% \toprule
%   &&\multicolumn{4}{c}{\textbf{FB15K-237}} & \multicolumn{4}{c}{\textbf{YAGO3-10}}\\
%   \cmidrule(l){3-6} \cmidrule(l){7-10}
%                     & $\mathcal{D}$ & MRR  & @1     &@3     & @10       & MRR  & @1 & @3 & @10\\
%   \toprule
%     DistMult        &train&0.253 &0.172   &0.283  &0.412     \\
%     \ac{SWA}   &&0.450 &0.334   &0.511  &0.675     \\
%     \approach  &&0.367 &0.262   &0.416  &0.571     \\
%     \midrule
%     DistMult        &val&0.159 &0.103   &0.175  &0.269      \\
%     \ac{SWA}          &&0.261 &0.182   &0.285  &0.422      \\
%     \approach         &&0.250 &0.180   &0.272  &0.389      \\
%     \midrule
%     DistMult       &test&0.158 &0.103   &0.173  &0.270      \\
%     \ac{SWA}             &&0.259 &0.179   &0.283  &0.422      \\
%     \approach         &&0.248 &0.178   &0.271  &0.390      \\
%     \midrule
%     \midrule
% \bottomrule
% \end{tabular}
% \end{table*}
% \begin{table*}
% \caption{Link prediction results on the train, validation and test splits of FB15K-237 and YAGO3-10. 
% Bold results indicate the best results.
% Num epochs 256, dim 32, batch size 1024 Adam with lr 0.1.}
% \label{table:fb15k_yago}
% \centering
% \small
% \begin{tabular}{l c c c c c c c c}
% \toprule
%   &\multicolumn{4}{c}{\textbf{FB15K-237}} & \multicolumn{4}{c}{\textbf{YAGO3-10}}\\
%   \cmidrule(l){2-5} \cmidrule(l){6-9}
%                     & MRR  & @1     &@3     & @10       & MRR  & @1 & @3 & @10\\
%   \toprule
%     DistMult-train   \\
%     \midrule
%     \midrule
%     \midrule
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}
% \caption{Link prediction results on the train, validation and test splits of FB15K-237 and YAGO3-10. 
% Bold results indicate the best results.
% Num epochs 128, dim 32, batch size 1024 Adam with lr 0.1.}
% \label{table:fb15k_yago}
% \centering
% \small
% \begin{tabular}{l c c c c c c c c}
% \toprule
%   &\multicolumn{4}{c}{\textbf{FB15K-237}} & \multicolumn{4}{c}{\textbf{YAGO3-10}}\\
%   \cmidrule(l){2-5} \cmidrule(l){6-9}
%                     & MRR  & @1     &@3     & @10       & MRR  & @1 & @3 & @10\\
%   \toprule
%     DistMult-train   \\
%     \midrule
%     \midrule
%     \midrule
% \bottomrule
% \end{tabular}
% \end{table*}




% \begin{table}[h]
% \caption{Link prediction results on the train, validation and test splits of FB15K-237 and YAGO3-10. Bold results indicate the best results.}
% \label{table:fb15k_yago}
% \centering
% \small
% \begin{tabular}{l c c c c c c c c}
% \toprule
%   &\multicolumn{4}{c}{\textbf{FB15K-237}} & \multicolumn{4}{c}{\textbf{YAGO3-10}}\\
%   \cmidrule(l){2-5} \cmidrule(l){6-9}
%       & MRR            & @1            & @3          & @10       & MRR  & @1 & @3 & @10\\
%   \toprule
%     DistMult-train  &0.991         &0.985&\textbf{0.999}&\textbf{1.000}&0.980&0.962&\textbf{0.998}&\textbf{1.000}\\
%     With \approach  &\textbf{0.994}&\textbf{0.990}&0.997&\textbf{1.000}&\textbf{0.981}&\textbf{0.963}&\textbf{0.998}&0.999\\
%     \midrule
%     DistMult-val    &0.124       &0.074       &0.132       &0.222 &0.400&0.337&0.433&0.520\\
%     With \approach  &\textbf{0.138}&\textbf{0.082}&\textbf{0.149}&\textbf{0.249}&\textbf{0.446}&\textbf{0.384}&\textbf{0.481}&\textbf{0.558}\\
%     \midrule
%     DistMult-test   &0.122      &0.071        &0.129      &0.223        &0.393&0.330&0.425&0.512\\
%     With \approach  &\textbf{0.134}&\textbf{0.080}&\textbf{0.145}&\textbf{0.243}&\textbf{0.441}&\textbf{0.377}&\textbf{0.481}&\textbf{0.558}\\
%     \midrule
%     \midrule
%     ComplEx-train    &0.995& 0.991&0.999&\textbf{1.000}&\textbf{0.984}&\textbf{0.969}&\textbf{1.000}&\textbf{1.000}\\
%     With \approach   &\textbf{0.996}&\textbf{0.993}&\textbf{1.000}&\textbf{1.000}&\textbf{0.984}&0.969&\textbf{1.000}&\textbf{1.000}\\
%     \midrule
%     ComplEx-val     &0.128&0.075&0.138&0.233&0.408&0.344&0.439&0.530\\
%     With \approach  &\textbf{0.153}&\textbf{0.095}&\textbf{0.169}&\textbf{0.270}&\textbf{0.444}&\textbf{0.378}&\textbf{0.484}&\textbf{0.562}\\
%     \midrule
%     Complex-test    &0.126&0.075&0.134&0.229&0.394&0.325&0.431&0.525\\
%     With \approach  &\textbf{0.150}&\textbf{0.094}&\textbf{0.165}&\textbf{0.264}&\textbf{0.433}&\textbf{0.366}&\textbf{0.473}&\textbf{0.554}\\
%     \midrule
%     \midrule
%     QMult-train    &0.989&0.981&0.997&0.999&0.821&0.790&0.841&0.877\\
%     With \approach &\textbf{0.995}&\textbf{0.990}&\textbf{1.000}&\textbf{1.000}&\textbf{0.828}&\textbf{0.792}&\textbf{0.852}&\textbf{0.881}\\
%     \midrule
%     QMult-val      &0.141       &0.083       &0.151       &0.258&0.306&0.241&0.338& 0.427\\
%     With \approach &\textbf{0.172}&\textbf{0.108}&\textbf{0.188}&\textbf{0.302}&\textbf{0.341}&\textbf{0.283}&\textbf{0.367}&\textbf{0.346}\\
%     \midrule
%     QMult-test     &0.138&0.082&0.146&0.253&0.300&0.232&0.334&0.424\\
%     With \approach &\textbf{0.167}&\textbf{0.102}&\textbf{0.183}&\textbf{0.298}&\textbf{0.339}&\textbf{0.282}&\textbf{0.365}&\textbf{0.444}\\
% \bottomrule
% \end{tabular}
% \end{table}

==> tables/nell.tex <==
\begin{table}[htb]
\caption{Link prediction results on the train, validation and test splits of NELL-995 h25 and  NELL-995 h50 benchmark datasets. Bold results indicate the best results.}
\centering
\small
%\resizebox{\columnwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
  &\multicolumn{4}{c}{\textbf{h25}} && \multicolumn{4}{c}{\textbf{h50}}\\
  \cmidrule(l){2-5} \cmidrule(l){7-10}
    & MRR & @1& @3 & @10              && MRR  & @1     & @3 & @10\\
  \toprule
    DistMult-train &\textbf{0.995}&0.991&0.998&\textbf{1.000}&&\textbf{0.955}&\textbf{0.934}&\textbf{0.974}&\textbf{0.990}&\\
    With \approach &\textbf{0.995}&\textbf{0.992}&\textbf{0.999}&\textbf{1.000}&& 0.895&0.863&0.921&0.951\\
    \midrule
DistMult-val  &0.151&0.107&0.164&0.235            &&0.162&0.114&0.178&\textbf{0.258}\\
With \approach&\textbf{0.159}&\textbf{0.116}&\textbf{0.172}&\textbf{0.240}&&\textbf{0.164}&\textbf{0.116}&\textbf{0.184}&0.257\\
    \midrule
DistMult-test &0.154&0.111&0.168&0.238&&0.164&0.116&0.116&0.257\\
With \approach&\textbf{0.162}&\textbf{0.119}&\textbf{0.177}&\textbf{0.245}            &&\textbf{0.166}&\textbf{0.119}&\textbf{0.184}&\textbf{0.258}\\
    \midrule
    \midrule
ComplEx-train &\textbf{1.000}&\textbf{1.000}&\textbf{1.000}&\textbf{1.000}&&0.991&0.986&0.995&0.996\\
With \approach&\textbf{1.000}&\textbf{1.000}&\textbf{1.000}&\textbf{1.000}&&\textbf{0.995}&\textbf{0.991}&\textbf{0.999}&\textbf{1.000}\\
    \midrule
ComplEx-val   &\textbf{0.105}&\textbf{0.069}&\textbf{0.110}&0.175&&0.079&0.048&0.082&0.143\\
With \approach&\textbf{0.105}&\textbf{0.069}&\textbf{0.110}&\textbf{0.176}&&\textbf{0.089}&\textbf{0.054}&\textbf{0.094}&\textbf{0.160}\\
    \midrule
Complex-test  &\textbf{0.106}&\textbf{0.071}&\textbf{0.110}&0.175&&0.080&0.049&0.085&0.141\\
With \approach&0.105&0.069&\textbf{0.110}&\textbf{0.178}&&\textbf{0.093}&\textbf{0.058}&\textbf{0.097}& \textbf{0.160}\\
    \midrule
    \midrule
QMult-train   &0.977&0.967&0.986&0.994                                          &&0.917&0.890&0.934&0.962\\
With \approach&\textbf{1.000}&\textbf{0.999}&\textbf{1.000}&\textbf{1.000}&&\textbf{0.924}&\textbf{0.902}&\textbf{0.937}&\textbf{0.966}\\
    \midrule
QMult-val     &0.084&0.055&0.090&0.140&&0.102&0.058&0.115&0.191\\
With \approach&\textbf{0.090}&\textbf{0.059}&\textbf{0.096}&\textbf{0.150}&&\textbf{0.114}&\textbf{0.068}&\textbf{0.127}&\textbf{0.206}\\
    \midrule
QMult-test    &0.081&0.052&0.086&0.138&&0.105&0.061&0.114&0.191\\
With \approach&\textbf{0.086}&\textbf{0.055}&\textbf{0.090}&\textbf{0.146}&&\textbf{0.116}&\textbf{0.070}&\textbf{0.126}&\textbf{0.211}\\
\bottomrule
\end{tabular}
%}
\label{table:nell}
\end{table}


==> tables/umls_kinship.tex <==
\begin{table}[htb]
    \centering
    \small
    \caption{Link prediction results on the train, validation and test splits of UMLS and KINSHIP benchmark datasets. Bold results indicate the best results.}
%    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l c c c c c c c c c c c c}
    \toprule
    &\multicolumn{4}{c}{\textbf{UMLS}} & \multicolumn{4}{c}{\textbf{KINSHIP}}\\
    \cmidrule(l){2-5} \cmidrule(l){6-9}
    &MRR             & @1  & @3  & @10  & MRR  & @1 & @3 & @10 &\\
  \toprule
DistMult-train   &0.992         &0.987         &0.997&\textbf{1.000} &0.847&0.781&0.893&0.977\\
With \approach&\textbf{0.999}&\textbf{0.998}&\textbf{0.999}&\textbf{1.000} &\textbf{0.865}&\textbf{0.806}&\textbf{0.906}&\textbf{0.981}\\
    \midrule
DistMult-val      &0.458&0.325&0.500&0.753 &0.399&0.256&0.432&0.741\\
With \approach    &\textbf{0.499}&\textbf{0.376}&\textbf{0.528}&\textbf{0.778}&\textbf{0.426}&\textbf{0.288}&\textbf{0.455}&\textbf{0.760}\\
    \midrule
DistMult-test     &0.450&0.321&0.491&0.755 &0.404&0.260&0.442&0.755\\
    With \approach    &\textbf{0.493}&\textbf{0.372}&\textbf{0.526}&\textbf{0.778}&\textbf{0.433}&\textbf{0.290}&\textbf{0.470}&\textbf{0.782}\\
    \midrule
    \midrule
ComplEx-train     &0.998&0.997&\textbf{1.000}&\textbf{1.000}&0.993&0.989&0.998&\textbf{1.000}\\
With \approach &\textbf{1.000}&\textbf{1.000}&\textbf{1.000}&\textbf{1.000}&\textbf{0.996}&\textbf{0.993}&\textbf{0.999}&\textbf{1.000}\\
    \midrule
ComplEx-val       &0.442&0.285&0.521&0.766&0.521&0.378&0.595&0.829\\
With \approach   &\textbf{0.491}&\textbf{0.350}&\textbf{0.550}&\textbf{0.783} &\textbf{0.599}&\textbf{0.463}&\textbf{0.677}&\textbf{0.861}\\
    \midrule
ComplEx-test      &0.444&0.287&0.528&0.773&0.533&0.388&0.614&0.821\\
With \approach  &\textbf{0.502}&\textbf{0.361}&\textbf{0.573}&\textbf{0.787}&\textbf{0.603}&\textbf{0.479}&\textbf{0.675}&\textbf{0.842}\\
    \midrule
    \midrule
    QMult-train       &0.998&0.998&0.999&0.999 &0.990&0.983&0.996&\textbf{0.999}\\
    With \approach    &\textbf{1.000}&\textbf{1.000}&\textbf{1.000}&\textbf{1.000}&\textbf{0.995}&\textbf{0.992}&\textbf{0.998}&\textbf{0.999}\\
    \midrule
    QMult-val        &0.445&0.280&0.524&0.791 &0.500&0.352&0.571&0.805\\
    With \approach   &\textbf{0.485}&\textbf{0.326}&\textbf{0.578}&\textbf{0.803} &\textbf{0.598}&\textbf{0.468}&\textbf{0.675}&\textbf{0.852}\\
    \midrule
    QMult-test       &0.426&0.272&0.498&0.757 &0.502&0.355&0.580&0.801\\
    With \approach &\textbf{0.480}&\textbf{0.334}&\textbf{0.555}&\textbf{0.786} &\textbf{0.591}&\textbf{0.467}&\textbf{0.668} & \textbf{0.838}\\
     \bottomrule
    \end{tabular}
\label{table:umls_kinship}
\end{table}
